How to Increase Interest in Studying Functional Programming via Interdisciplinary Application

Functional programming represents a modern tool for applying and implementing software. The state of the art in functional programming reports an increasing number of methodologies in this paradigm. However, extensive interdisciplinary applications are missing. Our goal is to increase student interest in pursuing further studies in functional programming with the use of an application: the ray tracer. We conducted a teaching experience, with positive results and student feedback, described here in this paper.

==> eptcsdata.tex <==
\providecommand{\firstpage}{37}
\providecommand{\publicationstatus}{J. Hage (Ed.): Trends in Functional Programming\\
in Education 2019 and 2020 (TFPIE '19 and '20)\\
EPTCS 321, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.321.3}{10.4204/EPTCS.321.3}}
\pdfoutput=1

